UniMorph 4.0: Universal Morphology

The Universal Morphology (UniMorph) project is a collaborative effort providing broad-coverage instantiated normalized morphological inflection tables for hundreds of diverse world languages. The project comprises two major thrusts: a language-independent feature schema for rich morphological annotation and a type-level resource of annotated data in diverse languages realizing that schema. This paper presents the expansions and improvements made on several fronts over the last couple of years (since McCarthy et al. (2020)). Collaborative efforts by numerous linguists have added 67 new languages, including 30 endangered languages. We have implemented several improvements to the extraction pipeline to tackle some issues, e.g. missing gender and macron information. We have also amended the schema to use a hierarchical structure that is needed for morphological phenomena like multiple-argument agreement and case stacking, while adding some missing morphological features to make the schema more inclusive. In light of the last UniMorph release, we also augmented the database with morpheme segmentation for 16 languages. Lastly, this new release makes a push towards inclusion of derivational morphology in UniMorph by enriching the data and annotation schema with instances representing derivational processes from MorphyNet.

==> tables/lang-descr.tex <==
%%Kat: Temporary put the table here 
%%This should probably go into Appendix + reformatted to fit the page + we need to add train/dev/test split size 
%% Sources should be moved to references
%% CODES Are ISO 639-3; Family/Genus -- based on WALS
\begin{table*}[ht]
\begin{adjustbox}{width=1\textwidth}
\small
\begin{tabular}{l|l|l|l|l}
%%DEVELOPMENT

\multicolumn{5}{l}{\textbf{Development}}\\
 Family & Genus & ISO 639-3 & Language & Source of Data \\
\toprule
Austronesian   &Barito   &mlg (plt)   &Malagasy    &\citet{malagasy} \\
    &Greater Central Philippine   &ceb   &Cebuano  & \citet{cebuano}            \\
    &Greater Central Philippine  &hil  & Hiligaynon  & \citet{hiligaynon} \\
    &Greater Central Philippine  &tgl   &Tagalog     & \citet{tagalog}     \\
    &Oceanic  &mao (mri)  & M\=aori      & \citet{maori}           \\
    \midrule
Indo-European  & Germanic   &ang   &Old English & \href{https://unimorph.github.io/}{UniMorph}\\
    &Germanic   &dan   &Danish & \href{https://unimorph.github.io/}{UniMorph} \\
    &Germanic    &deu   &German & \href{https://unimorph.github.io/}{UniMorph}\\
    &Germanic    &eng   &English& \href{https://unimorph.github.io/}{UniMorph}\\
    &Germanic    &frr   &North Frisian    & \href{https://unimorph.github.io/}{UniMorph}\\
    &Germanic    &gmh   & Middle High German      & \href{https://unimorph.github.io/}{UniMorph}\\
    &Germanic  &isl   & Icelandic & \href{https://unimorph.github.io/}{UniMorph}\\
    &Germanic    &nld   &Dutch& \href{https://unimorph.github.io/}{UniMorph} \\
    &Germanic     &nob   &Norwegian Bokmål      & \href{https://unimorph.github.io/}{UniMorph}\\
    &Germanic     &swe   &Swedish      & \href{https://unimorph.github.io/}{UniMorph}\\
    \midrule
Niger-Congo &Bantoid   &kon (kng)   &Kongo& \citet{kongo}  \\
    &Bantoid    &lin   &Lingala & \citet{lingala}\\
    &Bantoid   &lug   &Luganda     &\citet{luganda}\\
    &Bantoid    &nya   &Chewa  & \citet{chewa}\\
    &Bantoid &sot   &Sotho & \citet{sotho}         \\
    &Bantoid    &swa (swh)   & Swahili &\citet{swahili}    \\
    &Bantoid    &zul   &Zulu      & \citet{zulu}       \\
    &Kwa   &aka   &Akan & \citet{akan} \\
    &Kwa   &gaa   &Gã       & \citet{ga} \\
    \midrule
Oto-Manguean    &Amuzgoan  &azg   &San Pedro Amuzgos Amuzgo      & \citet{azg2015}        \\
    &Chichimec  &pei   &Chichimeca-Jonaz      & \citet{pei2015}     \\
    &Chinantecan   &cpa  &Tlatepuzco Chinantec       & \citet{cpa2015}         \\
    &Mixtecan   &xty   &Yoloxóchitl Mixtec      & \citet{xty2015}            \\
    &Otomian   &ote   &Mezquital Otomi  & \citet{ote2015}            \\
    &Otomian  &otm   &Sierra Otomi  & \citet{otm2015}    \\
    &Zapotecan    &cly   &Eastern Chatino of San Juan Quiahije &    \citet{cruz-anastasopoulos-stump:2020:LREC}    \\
    &Zapotecan &ctp   & Eastern Chatino of Yaitepec   & \citet{ctp2015}     \\
    &Zapotecan  &czn   &Zenzontepec Chatino  & \citet{czn2015}          \\
    &Zapotecan    &zpv   &Chichicapan Zapotec      & \citet{zpv2015}     \\
    \midrule
Uralic    &Finnic    &est   &Estonian   & \href{https://unimorph.github.io/}{UniMorph}          \\
    &Finnic    &fin   &Finnish     & \href{https://unimorph.github.io/}{UniMorph}           \\
    &Finnic    &izh   &Ingrian      & \href{https://unimorph.github.io/}{UniMorph}            \\
    &Finnic   &krl   &Karelian     &\citet{zaytseva2017open}  \\
    &Finnic  &liv   &Livonian       & \href{https://unimorph.github.io/}{UniMorph}           \\
    &Finnic   &vep   &Veps  &\citet{zaytseva2017open}  \\
    &Finnic   &vot   &Votic  & \href{https://unimorph.github.io/}{UniMorph}\\
    &Mari   &mhr   &Meadow Mari    &\citet{arkhangeskiy2012creation}\\
    &Mordvin    &mdf   &Moksha     &\citet{arkhangeskiy2012creation}\\
    &Mordvin    &myv   &Erzya    &\citet{arkhangeskiy2012creation} \\
    &Saami   &sme   &Northern Sami       & \href{https://unimorph.github.io/}{UniMorph}   \\      
\end{tabular}
\end{adjustbox}
\caption{Development languages used in the shared task.}
\label{tab:lang-descr}
\end{table*}

==> tables/lang-descr2.tex <==
\begin{table*}[!ht]
\begin{adjustbox}{width=1\textwidth}
\small
\begin{tabular}{l|l|l|l|l}
%%SURPRISE
\multicolumn{5}{l}{\textbf{Development}}\\
 Family & Genus & ISO 639-3 & Language & Source of Data \\
\toprule
 Afro-Asiatic & Semitic & mlt & Maltese & \href{https://unimorph.github.io/}{UniMorph} \\
& Lowland East Cushitic & orm & Oromo& \citet{oromo}  \\
 & Semitic & syc & Syriac & \href{https://unimorph.github.io/}{UniMorph} \\
\midrule
 Algic & Algonquian& cre & Plains Cree & \citet{cree} \\
 \midrule
 Tungusic & Tungusic & evn & Evenki & \citet{klyachko2020lowresourceeval}  \\
 \midrule
  Turkic & Turkic & aze (azb) & Azerbaijani & \href{https://unimorph.github.io/}{UniMorph}\\
  & Turkic & bak & Bashkir&  \href{https://unimorph.github.io/}{UniMorph}  \\
  & Turkic & crh & Crimean Tatar &  \href{https://unimorph.github.io/}{UniMorph} \\
  & Turkic & kaz & Kazakh & \citet{kazakh,kazakh2}  \\
  & Turkic  & kir & Kyrgyz & \citet{kyrgyz}   \\
  & Turkic & kjh & Khakas & \href{https://unimorph.github.io/}{UniMorph}\\
  & Turkic & tuk & Turkmen & \citet{turkmen,turkmen2}  \\
    & Turkic & uig & Uyghur & \citet{uyghur}  \\
    & Turkic & uzb & Uzbek & \citet{uzbek,uzbek2}   \\
    \midrule
 Dravidian & Southern Dravidian & kan & Kannada & \href{https://unimorph.github.io/}{UniMorph} \\
        &South-Central Dravidian& tel & Telugu & \href{https://unimorph.github.io/}{UniMorph}     \\
        \midrule
 Indo-European  & Indic & ben & Bengali & \href{https://unimorph.github.io/}{UniMorph}\\
    & Indic & hin & Hindi & \href{https://unimorph.github.io/}{UniMorph}  \\
    & Indic & san & Sanskrit & \href{https://unimorph.github.io/}{UniMorph}\\
    & Indic & urd & Urdu& \href{https://unimorph.github.io/}{UniMorph}\\
    & Iranian & fas (pes) & Persian & \href{https://unimorph.github.io/}{UniMorph} \\
    & Iranian & pus (pst) & Pashto & \href{https://unimorph.github.io/}{UniMorph} \\
    & Iranian & tgk & Tajik& \href{https://unimorph.github.io/}{UniMorph} \\
    & Romance & ast & Asturian & \href{https://unimorph.github.io/}{UniMorph} \\
    & Romance & cat & Catalan & \href{https://unimorph.github.io/}{UniMorph} \\
    & Romance & frm & Middle French & \href{https://unimorph.github.io/}{UniMorph}\\
    & Romance & fur & Friulian& \href{https://unimorph.github.io/}{UniMorph}\\
    & Romance & glg & Galician & \href{https://unimorph.github.io/}{UniMorph} \\
    & Romance & lld & Ladin & \href{https://unimorph.github.io/}{UniMorph} \\
    & Romance & vec & Venetian & \href{https://unimorph.github.io/}{UniMorph} \\
    & Romance & xno & Anglo-Norman & \href{https://unimorph.github.io/}{UniMorph}  \\
   & West Germanic & gml & Middle Low German & \href{https://unimorph.github.io/}{UniMorph} \\
    & West Germanic & gsw &Swiss German & \citet{ch}\\
    & North Germanic & nno & Norwegian Nynorsk & \href{https://unimorph.github.io/}{UniMorph} \\
 \midrule
 Niger-Congo & Bantoid & sna & Shona & \citet{shona,shona2} \\
 \midrule
Sino-Tibetan & Bodic & bod & Tibetan & \citet{di2019modelling} \\
\midrule
 Siouan & Core Siouan & dak  & Dakota & \citet{dakota}  \\
 \midrule
 Songhay & Songhay & dje &Zarma& \citet{zarma}\\
 \midrule
 Southern Daly & Murrinh-Patha & mwf & Murrinh-Patha & \citet{mansfield2019murrinhpatha}\\
 \midrule
 Uralic & Permic & kpv & Komi-Zyrian & \citet{arkhangeskiy2012creation}  \\
    & Finnic & lud & Ludic& \citet{zaytseva2017open}  \\
    & Finnic & olo & Livvi & \citet{zaytseva2017open} \\
    & Permic & udm & Udmurt & \citet{arkhangeskiy2012creation}  \\
    & Finnic & vro & V\~{o}ro & \citet{iva2007voru}\\
    \midrule
 Uto-Aztecan & Tepiman & ood & O'odham  &   \citet{oodham}
\end{tabular}
\end{adjustbox}
\caption{Surprise languages used in the shared task.}
\label{tab:lang-descr2}
\end{table*}

